Curriculum Prompting Foundation Models for Medical Image Segmentation

Adapting large pre-trained foundation models, e.g., SAM, for medical image segmentation remains a significant challenge. A crucial step involves the formulation of a series of specialized prompts that incorporate specific clinical instructions. Past works have been heavily reliant on a singular type of prompt for each instance, necessitating manual input of an ideally correct prompt, which is less efficient. To tackle this issue, we propose to utilize prompts of different granularity, which are sourced from original images to provide a broader scope of clinical insights. However, combining prompts of varying types can pose a challenge due to potential conflicts. In response, we have designed a coarse-to-fine mechanism, referred to as curriculum prompting, that progressively integrates prompts of different types. Through extensive experiments on three public medical datasets across various modalities, we demonstrate the effectiveness of our proposed approach, which not only automates the prompt generation process but also yields superior performance compared to other SAM-based medical image segmentation methods. Code is available at: https://github.com/AnnaZzz-zxq/Curriculum-Prompting.

==> RelatedWorks.tex <==
\section{Related Works}
\subsection{Segment Anything Model}
\subsection{Object Detection and Keypoint Detection Networks}
\subsection{Curriculum Learning}


==> TrainingTimeTable.tex <==

% \begin{table}[]
% \centering
% \renewcommand\arraystretch{1.2}
% \caption{Training times on three datasets.}\label{tab4}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{clclclclclc}
% \toprule[1pt] 
% \multicolumn{1}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{4}{c}{Curriculum Prompting}      & \multicolumn{1}{c}{\multirow{2}{*}{nnSAM}} \\
% \multicolumn{1}{c|}{}                         & Grounding DINO & HRNet & SAM(box) & SAM(mask) & \multicolumn{1}{c}{}                       \\
% \multicolumn{1}{l|}{TN3K}                     & 2h             & 2h    & 4h       & 1.5h      & 15.2h                                      \\ \cline{1-1}
% \multicolumn{1}{l|}{Kvasir}                   & 50min          & 40min & 1h       & 20min     & 12.5h                                      \\ \cline{1-1}
% QaTa-COV19                                    & 6h             & 6h    & 6.7h     & 2.6h      & 20.8h   \\                              \bottomrule[1pt]    
% \end{tabular}%
% }
% \end{table}


\begin{table}[h]
\centering
\renewcommand\arraystretch{1.2}
\caption{Training times on three datasets.}\label{tab4}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule[1pt]
\multirow{2}{*}{Dataset} & \multicolumn{4}{c}{Curriculum Prompting} & \multirow{2}{*}{nnSAM} \\ \cline{2-5}
                         & Grounding DINO & HRNet & SAM(box) & SAM(mask) & \\ \midrule[1pt]
TN3K                     & 2h             & 2h    & 4h       & 1.5h      & 15.2h  \\
Kvasir                   & 50min          & 40min & 1h       & 20min     & 12.5h  \\
QaTa-COV19               & 6h             & 6h    & 6.7h     & 2.6h      & 20.8h  \\ \bottomrule[1pt]
\end{tabular}%
}
\end{table}

